MMDocBench: Benchmarking Large Vision-Language Models for Fine-Grained Visual Document Understanding

Large Vision-Language Models (LVLMs) have achieved remarkable performance in many vision-language tasks, yet their capabilities in fine-grained visual understanding remain insufficiently evaluated. Existing benchmarks either contain limited fine-grained evaluation samples that are mixed with other data, or are confined to object-level assessments in natural images. To holistically assess LVLMs' fine-grained visual understanding capabilities, we propose using document images with multi-granularity and multi-modal information to supplement natural images. In this light, we construct MMDocBench, a benchmark with various OCR-free document understanding tasks for the evaluation of fine-grained visual perception and reasoning abilities. MMDocBench defines 15 main tasks with 4,338 QA pairs and 11,353 supporting regions, covering various document images such as research papers, receipts, financial reports, Wikipedia tables, charts, and infographics. Based on MMDocBench, we conduct extensive experiments using 13 open-source and 3 proprietary advanced LVLMs, assessing their strengths and weaknesses across different tasks and document image types. The benchmark, task instructions, and evaluation code will be made publicly available.

==> fig_tree.tex <==

%  \begin{figure}
%     \centering
    
% % I am using only the basic, xnode, and tnode styles
% \tikzset{
%     basic/.style  = {fill=green!10, text width=2.3cm},
%     root/.style   = {basic, rounded corners=2pt, thin, align=left, fill=green!30},
%     onode/.style = {basic, thin, rounded corners=2pt, align=left, fill=blue!30,text width=2.3cm,font=\small},
%     tnode/.style = {basic, thin, fill=pink!60, text width=2.3cm, align=left, font=\small},
%     xnode/.style = {draw, thick, rounded corners=2pt, align=left, fill=gray!20,text width=2.3cm ,draw, font=\small},
%     wnode/.style = {basic, thin, align=center, fill=pink!10!blue!80!red!10, text width=6.5em, fill=white},
%     edge from parent/.style={draw=black, thin, edge from parent fork right,}
% }
% %

% \begin{forest} for tree={
%     grow=east,
%     growth parent anchor=west,
%     parent anchor=east,
%     child anchor=west,
%     base=left,
%     font=\small,
%     rectangle,
%     draw,
%     rounded corners,
%     align=left,
%     minimum width=2.5em,
%     inner xsep=4pt,
%     inner ysep=1pt
% }
% % l sep is used for arrow distance
% [\bench, basic, wnode 
%     [Visual Reasoning, tnode,  l sep=6mm,
%         [Arithmetic Reasoning, tnode]
%         [Arithmetic Reasoning, tnode]
%         [Arithmetic Reasoning, tnode] 
%         [Arithmetic Reasoning, tnode] 
%         [Arithmetic Reasoning, tnode] 
%         [Arithmetic Reasoning, tnode,
%          [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]] 
%         ]
%     [Visual Perception, onode, l sep=6mm,
%         [Infographic QA, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Chart QA, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Document  QA, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Document Forgery Detection, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Key Information Extraction, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Table  Cell Localization, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Text  Localization, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Table Recognition, onode, 
%         [Flickr30k Entities\cite{2023GPT4VisionSC}; \\
%             Visual7W\cite{2023GPT4VisionSC}, xnode]]
%         [Text Recognition, onode, 
%         [
%             Flickr30k Entities\cite{2023GPT4VisionSC};\\
%             Visual7W\cite{2023GPT4VisionSC};, xnode]
%         ]
%     ]]
% \end{forest}

%     \caption{Literature Survey Tree}
%     \label{fig:lit_surv}
% \end{figure}




% \begin{figure}
%     \centering

% % I am using only the basic, xnode, and tnode styles
% \tikzset{
%     basic/.style  = {fill=green!10, text width=2.2cm, align=center, font=\small},
%     root/.style   = {basic, rounded corners=2pt, thin, align=left, fill=green!30,font=\small},
%     onode/.style = {basic, thin, rounded corners=2pt, align=left, fill=blue!20, text width=2.3cm, font=\small},
%     tnode/.style = {basic, thin, align=left, fill=pink!60, text width=7em, align=left,font=\small},
%     xnode/.style = {basic, thin, rounded corners=2pt, align=left, fill={rgb:red,54;green,94;yellow,186}, text width=3cm},
%     wnode/.style = {basic, thin, align=left, fill=pink!10!blue!80!red!10, text width=3em},
%     edge from parent/.style={draw=black, edge from parent fork right}

% }
% %

% \begin{forest} for tree={
%     grow=east,
%     growth parent anchor=west,
%     parent anchor=east,
%     child anchor=west,
%     edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
%          (!u.parent anchor) -- +(10pt,0pt) |-  (.child anchor) 
%          \forestoption{edge label};}
% }

% % l sep is used for arrow distance
% [\bench, basic,  l sep=8mm,
%     [Visual Reasoning, onode,  l sep=8mm,
%         [Chiew et al.\, 2018, tnode]
%         [Heartfield \& Loukas\, 2015, tnode]
%         [Salahdine et al.\, 2019, tnode] 
%         [Alharthi et al.\, 2020, tnode] ]
%     [Visual Perception, onode, l sep=8mm,
%         [Infographic QA, tnode]
%         [Chart QA, tnode]
%         [Document QA, tnode]
%     ]
   
%    ]
% \end{forest}

%     \caption{Literature Survey Tree}
%     \label{fig:lit_surv}
% \end{figure}


